Data Provenance Auditing of Fine-Tuned Large Language Models with a Text-Preserving Technique

We propose a system for marking sensitive or copyrighted texts to detect their use in fine-tuning large language models under black-box access with statistical guarantees. Our method builds digital ``marks'' using invisible Unicode characters organized into (``cue'', ``reply'') pairs. During an audit, prompts containing only ``cue'' fragments are issued to trigger regurgitation of the corresponding ``reply'', indicating document usage. To control false positives, we compare against held-out counterfactual marks and apply a ranking test, yielding a verifiable bound on the false positive rate. Empirically, we obtain a true positive rate of 96.7% at 0% false positive rate and reply regurgitation rates exceeding 28% per document with only 40 (4%) watermarked documents. The approach is minimally invasive, scalable across many sources, robust to standard processing pipelines, and achieves high detection power even when marked data is a small fraction of the fine-tuning corpus.

==> includes/img/H2_figure.tex <==
% blog1k - mistral
\pgfplotstableread[row sep=\\,col sep=space]{
model    nbdocs   c1      c2      c3      c4      c5 \\
mistral  10       0       0       0       0       0 \\
mistral  20       0.05    0.05    0       0       0 \\
mistral  30       0.10    0.2333  0.20    0.0667  0.10 \\
mistral  40       0.375   0.35    0.15    0.40    0.225 \\
mistral  50       0.54    0.62    0.70    0.58    0.50 \\
mistral  60       0.6333  0.5167  0.6333  0.4667  0.5333 \\
mistral  70       0.6571  0.7286  0.70    0.7286  0.70 \\
mistral  80       0.8875  0.825   0.8875  0.85    0.95 \\
mistral  90       0.9444  0.8889  0.9667  0.9667  0.9556 \\
mistral  100      0.97    0.97    0.97    0.94    0.95 \\
}\blogMistral

% blog1k - llama
\pgfplotstableread[row sep=\\,col sep=space]{
model    nbdocs   c1      c2      c3      c4      c5 \\
llama    10       0       0       0       0       0 \\
llama    20       0       0       0.05    0.15    0.10 \\
llama    30       0.6667  0.7333  0.8333  0.7333  0.7667 \\
llama    40       0.825   0.875   0.925   0.875   0.925 \\
llama    50       0.86    0.94    0.96    0.94    0.96 \\
llama    60       0.8833  0.95    0.9667  0.95    0.9667 \\
llama    70       0.9571  0.9714  0.9857  0.9714  0.9857 \\
llama    80       0.9875  0.95    0.95    0.9625  0.9875 \\
llama    90       0.9778  0.9667  0.9889  0.9889  1.0 \\
llama    100      0.97    0.95    0.96    0.96    0.96 \\
}\blogLlama

% poem - mistral
\pgfplotstableread[row sep=\\,col sep=space]{
model    nbdocs   c1      c2      c3      c4      c5 \\
mistral  10       0       0       0       0       0 \\
mistral  20       0       0       0       0       0 \\
mistral  30       0       0       0       0       0 \\
mistral  40       0.025   0.05    0.05    0       0.025 \\
mistral  50       0.20    0.12    0.10    0.14    0.10 \\
mistral  60       0.30    0.25    0.2167  0.2167  0.2167 \\
mistral  70       0.4714  0.4571  0.4286  0.4429  0.3571 \\
mistral  80       0.525   0.40    0.4375  0.5375  0.425 \\
mistral  90       0.90    0.9222  0.9444  0.9111  0.9444 \\
mistral  100      0.94    0.93    0.97    0.89    0.93 \\
}\poemMistral

% poem - llama
\pgfplotstableread[row sep=\\,col sep=space]{
model    nbdocs   c1      c2      c3      c4      c5 \\
llama  10       0       0       0       0       0 \\
llama  20       0       0       0       0       0 \\
llama  30       0.1333  0.30    0.2667  0.20    0.3667 \\
llama  40       0.65    0.725   0.80    0.725   0.675 \\
llama  50       0.88    0.78    0.84    0.76    0.80 \\
llama  60       0.9333  0.9333  0.9333  0.90    0.9333 \\
llama  70       0.9429  0.9286  0.9571  0.9571  0.9286 \\
llama  80       1.0     0.925   0.9875  0.9625  0.95 \\
llama  90       1.0     0.9556  0.9667  0.9111  0.9667 \\
llama  100      0.99    0.97    0.98    0.96    0.98 \\
}\poemLlama

% ====== calculate avg and std in ratio space ======
\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\blogMistral}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\blogMistral}

\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\blogLlama}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\blogLlama}

\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\poemMistral}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\poemMistral}

\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\poemLlama}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\poemLlama}

\renewcommand{\plotwidth}{8.5cm}
\newcommand{\plotheight}{7cm}
\begin{figure}
  \centering
    \begin{tikzpicture}
    
    % ========= avg + legend =========
    \begin{axis}[
      name=main,
      width=\plotwidth, height=\plotheight,
      xlabel={Number of watermarked documents},
      ylabel={Number of regurgitated replies},
      ytick={0,10,...,100},
      ymin=0, ymax=105,
      xmin=0, xmax=100,
      legend style={at={(1.00,0.02)}, anchor=south east, font=\scriptsize, draw=none, fill=none},
      nodes={scale=0.8, transform shape},
      legend image post style={mark options={fill=.,draw=.}}
    ]
    
    % ---- blog - mistral
    \addplot+[color=blogColor, thick, solid, mark=*]
      table[x=nbdocs,y expr=\thisrow{avgRatio}*\thisrow{nbdocs}]{\blogMistral};
    \addlegendentry{mistral --- blog1k}
    
    % ---- blog - llama
    \addplot+[color=blogColor, thick, dashed, mark=square*,
              mark options={fill=blogColor, draw=blogColor}]
      table[x=nbdocs,y expr=\thisrow{avgRatio}*\thisrow{nbdocs}]{\blogLlama};
    \addlegendentry{llama --- blog1k}
    
    % ---- poem - mistral
    \addplot+[color=poemColor, thick, solid, mark=triangle*,
              mark options={fill=poemColor, draw=poemColor}]
      table[x=nbdocs,y expr=\thisrow{avgRatio}*\thisrow{nbdocs}]{\poemMistral};
    \addlegendentry{mistral --- poem}
    
    % ---- poem - llama
    \addplot+[color=poemColor, thick, dashed, mark=star]
      table[x=nbdocs,y expr=\thisrow{avgRatio}*\thisrow{nbdocs}]{\poemLlama};
    \addlegendentry{llama --- poem}
    
    \end{axis}
    
    % ========= std (shaded areas) =========
    \begin{axis}[
      at={(main.south west)}, anchor=south west,
      width=\plotwidth, height=\plotheight,
      xmin=0, xmax=100,
      ymin=0, ymax=105,
      axis line style={draw=none},
      tick style={draw=none},
      xticklabels=\empty,
      yticklabels=\empty,
      legend=false
    ]
    
    % blog1k - mistral 
    \addplot[name path=upperA,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*\thisrow{nbdocs}]{\blogMistral};
    \addplot[name path=lowerA,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*\thisrow{nbdocs}]{\blogMistral};
    \addplot[blogColor!30,fill opacity=0.5,forget plot]
      fill between[of=upperA and lowerA];
    
    % blog1k - llama 
    \addplot[name path=upperB,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*\thisrow{nbdocs}]{\blogLlama};
    \addplot[name path=lowerB,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*\thisrow{nbdocs}]{\blogLlama};
    \addplot[blogColor!30,fill opacity=0.5,forget plot]
      fill between[of=upperB and lowerB];
    
    % poem - mistral 
    \addplot[name path=upperC,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*\thisrow{nbdocs}]{\poemMistral};
    \addplot[name path=lowerC,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*\thisrow{nbdocs}]{\poemMistral};
    \addplot[poemColor!30,fill opacity=0.5,forget plot]
      fill between[of=upperC and lowerC];
    
    % poem - llama 
    \addplot[name path=upperD,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*\thisrow{nbdocs}]{\poemLlama};
    \addplot[name path=lowerD,draw=none]
      table[x=nbdocs,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*\thisrow{nbdocs}]{\poemLlama};
    \addplot[poemColor!30,fill opacity=0.5,forget plot]
      fill between[of=upperD and lowerD];
    
    \end{axis}
    
    \end{tikzpicture}
    
    \caption{Number of regurgitated replies depending on collection size. Curves show average regurgitated replies; shaded areas indicate $\pm$ standard deviation.}
    \label{fig:h2-results}
\end{figure}






==> includes/tables/H2_table.tex <==
\begin{table}
\centering
\caption{Empirical estimation of $p$ and $p_{FN}$ .}
\label{tab:success-residual}
\begin{subtable}{\columnwidth}
\centering
\caption{Blog1k}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}{*}{nbdocs} & \multicolumn{2}{c|}{Mistral} & \multicolumn{2}{c}{LLaMA} \\
 & $p$ & $p_{FN}$ & $p$ & $p_{FN}$ \\
\hline
% 10  & 0.000 & 1.000 & 0.000 & 1.000 \\
% 20  & 0.020 & 0.668 & 0.060 & 0.294 \\
30  & 0.140 & 0.0108 & 0.747 & 3.0$\times 10^{-5}$ \\
40  & 0.300 & 6.4$\times 10^{-7}$ & 0.885 & 4.5$\times 10^{-21}$ \\
50  & 0.588 & 5.6$\times 10^{-20}$ & 0.940 & 7.7$\times 10^{-42}$ \\
% 60  & 0.557 & 6.4$\times 10^{-22}$ & 0.940 & 1.2$\times 10^{-41}$ \\
% 70  & 0.703 & 1.3$\times 10^{-37}$ & 0.974 & 1.1$\times 10^{-89}$ \\
% 80  & 0.880 & 2.2$\times 10^{-74}$ & 0.968 & 3.0$\times 10^{-76}$ \\
% 90  & 0.944 & 1.0$\times 10^{-113}$ & 0.984 & 1.5$\times 10^{-140}$ \\
% 100 & 0.960 & 1.6$\times 10^{-140}$ & 0.960 & 1.6$\times 10^{-140}$ \\
\hline
\end{tabular}
}
\end{subtable}

\vspace{0.4cm}

\begin{subtable}{\columnwidth}
\centering
\caption{Poems}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}{*}{nbdocs} & \multicolumn{2}{c|}{Mistral} & \multicolumn{2}{c}{LLaMA} \\
 & $p$ & $p_{FN}$ & $p$ & $p_{FN}$ \\
\hline
% 10  & 0.000 & 1.000 & 0.000 & 1.000 \\
% 20  & 0.000 & 1.000 & 0.000 & 1.000 \\
30  & 0.000 & 1.000 & 0.253 & 5.8$\times 10^{-5}$ \\
40  & 0.030 & 0.305 & 0.715 & 1.9$\times 10^{-9}$ \\
50  & 0.132 & 9.4$\times 10^{-4}$ & 0.812 & 1.1$\times 10^{-22}$ \\
% 60  & 0.242 & 1.0$\times 10^{-4}$ & 0.927 & 3.4$\times 10^{-44}$ \\
% 70  & 0.431 & 1.8$\times 10^{-8}$ & 0.943 & 1.3$\times 10^{-57}$ \\
% 80  & 0.465 & 6.1$\times 10^{-15}$ & 0.965 & 2.1$\times 10^{-88}$ \\
% 90  & 0.924 & 4.7$\times 10^{-6}$ & 0.960 & 2.0$\times 10^{-70}$ \\
% 100 & 0.932 & 1.8$\times 10^{-7}$ & 0.976 & 5.0$\times 10^{-105}$ \\
\hline
\end{tabular}
}
\end{subtable}
\end{table}


==> includes/tables/H3_figure.tex <==


\pgfplotstableread[row sep=\\,col sep=space]{
model    trainset   c1      c2      c3      c4      c5 \\
llama    1000       0.825   0.875   0.925   0.875   0.925 \\
llama    5000       0.925   0.925   0.900   0.825   0.950 \\
llama    10000      0.975   0.775   0.925   0.850   0.925 \\
llama    15000      0.925   0.900   0.950   0.925   0.950 \\
}\blogLlama

\pgfplotstableread[row sep=\\,col sep=space]{
model    trainset   c1      c2      c3      c4      c5 \\
mistral  1000       0.540   0.620   0.700   0.580   0.500 \\
mistral  5000       0.540   0.520   0.500   0.520   0.460 \\
mistral  10000      0.680   0.700   0.700   0.620   0.560 \\
mistral  15000      0.560   0.480   0.320   0.400   0.500 \\
}\blogMistral

\pgfplotstableread[row sep=\\,col sep=space]{
model    trainset   c1      c2      c3      c4      c5 \\
llama    1000       0.650   0.725   0.800   0.725   0.675 \\
llama    2500       0.800   0.600   0.825   0.775   0.750 \\
llama    5000       0.525   0.625   0.725   0.625   0.750 \\
}\poemLlama

\pgfplotstableread[row sep=\\,col sep=space]{
model    trainset   c1      c2      c3      c4      c5 \\
mistral  1000       0.300   0.250   0.2167  0.2167  0.2167 \\
mistral  2500       0.150   0.2333  0.2167  0.2333  0.1667 \\
mistral  5000       0.4333  0.3667  0.3167  0.3333  0.300 \\
}\poemMistral

% ==========  avg and std ==========
% --- Blog LLaMA ---
\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\blogLlama}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\blogLlama}

% --- Blog Mistral ---
\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\blogMistral}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\blogMistral}

% --- Poem LLaMA ---
\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\poemLlama}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\poemLlama}

% --- Poem Mistral ---
\pgfplotstablecreatecol[
  create col/expr={( (\thisrow{c1}+\thisrow{c2}+\thisrow{c3}+\thisrow{c4}+\thisrow{c5})/5 )}
]{avgRatio}{\poemMistral}
\pgfplotstablecreatecol[
  create col/expr={sqrt(( (\thisrow{c1}-\thisrow{avgRatio})^2
                        +(\thisrow{c2}-\thisrow{avgRatio})^2
                        +(\thisrow{c3}-\thisrow{avgRatio})^2
                        +(\thisrow{c4}-\thisrow{avgRatio})^2
                        +(\thisrow{c5}-\thisrow{avgRatio})^2 )/5)}
]{stdRatio}{\poemMistral}







\begin{figure}
\centering

% ====== Blog ======
\begin{subfigure}{0.48\linewidth}
  \begin{tikzpicture}
    \begin{axis}[
      width=\linewidth, height=6cm,
      xlabel={Training set size},
      ylabel={Number of regurgitated replies},
      ymin=0, ymax=55,
      ytick={0,10,...,50},
      scaled x ticks=false,
      xtick={1000,5000,10000,15000},
      xticklabels={1k,5k,10k,15k},
      xticklabel style={/pgf/number format/fixed},
      legend style={at={(0.98,0.02)}, anchor=south east, font=\scriptsize, draw=none, fill=none}
    ]
      % mistral (50 docs)
      \addplot+[poemColor, thick, solid, mark=*, mark options={fill=poemColor, draw=poemColor}]
        table[x=trainset,y expr=\thisrow{avgRatio}*50]{\blogMistral};
      \addlegendentry{Mistral}

      % llama (40 docs)
      \addplot+[poemColor, thick, dashed, mark=square*, mark options={fill=poemColor, draw=poemColor}]
        table[x=trainset,y expr=\thisrow{avgRatio}*40]{\blogLlama};
      \addlegendentry{LLaMA}

      % shading mistral
      \addplot[name path=upperA,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*50]{\blogMistral};
      \addplot[name path=lowerA,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*50]{\blogMistral};
      \addplot[poemColor!30,fill opacity=0.5,forget plot] fill between[of=upperA and lowerA];

      % shading llama
      \addplot[name path=upperB,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*40]{\blogLlama};
      \addplot[name path=lowerB,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*40]{\blogLlama};
      \addplot[poemColor!30,fill opacity=0.5,forget plot] fill between[of=upperB and lowerB];
    \end{axis}
  \end{tikzpicture}
  \caption{Blog1k dataset}
  \label{fig:h3-results-blog}
\end{subfigure}
\hfill
% ====== Poem ======
\begin{subfigure}{0.48\linewidth}
  \begin{tikzpicture}
    \begin{axis}[
      width=\linewidth, height=6cm,
      xlabel={Training set size},
      ylabel={Number of regurgitated replies},
      ymin=0, ymax=65,
      ytick={0,10,...,60},
      legend style={at={(0.98,0.02)}, anchor=south east, font=\scriptsize, draw=none, fill=none}
    ]
      % mistral (60 docs)
      \addplot+[blogColor, thick, solid, mark=triangle*, mark options={fill=blogColor, draw=blogColor}]
        table[x=trainset,y expr=\thisrow{avgRatio}*60]{\poemMistral};
      \addlegendentry{Mistral}

      % llama (40 docs)
      \addplot+[blogColor, thick, dashed, mark=star]
        table[x=trainset,y expr=\thisrow{avgRatio}*40]{\poemLlama};
      \addlegendentry{LLaMA}

      % shading mistral
      \addplot[name path=upperC,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*60]{\poemMistral};
      \addplot[name path=lowerC,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*60]{\poemMistral};
      \addplot[blogColor!30,fill opacity=0.5,forget plot] fill between[of=upperC and lowerC];

      % shading llama
      \addplot[name path=upperD,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}+\thisrow{stdRatio})*40]{\poemLlama};
      \addplot[name path=lowerD,draw=none]
        table[x=trainset,y expr=(\thisrow{avgRatio}-\thisrow{stdRatio})*40]{\poemLlama};
      \addplot[blogColor!30,fill opacity=0.5,forget plot] fill between[of=upperD and lowerD];
of    \end{axis}
  \end{tikzpicture}
  \caption{Poem dataset}
  \label{fig:h3-results-poem}
\end{subfigure}

\caption{Average regurgitated replies with $\pm$ std across varying dataset sizes with fixed collection size. Left: Blog1k ($\col$ size: Mistral=50, LLaMA=40). Right: Poems ($\col$ size: Mistral=60, LLaMA=40). Solid = Mistral, dashed = LLaMA.{\color{red}Lorena comment: I would use the same scale in all plts of the same type to allow fair comparisons}}
\end{figure}

